Improving the Diproche CNL through Autoformalization via Large Language Models

The Diproche system is an automated proof checker for texts written in a controlled fragment of German, designed for didactical applications in classes introducing students to proofs for the first time. The first version of the system used a controlled natural language for which a Prolog formalization routine was written. In this paper, we explore the possibility of prompting large language models for autoformalization in the context of Diproche, with encouraging first results.

==> eptcsdata.tex <==
\providecommand{\firstpage}{44}
\providecommand{\publicationstatus}{J. Narboux, W. Neuper and P. Quaresma (Eds.): Workshop on\\ Theorem proving components for Educational software 2023 (ThEdu'23)\\
EPTCS 400, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.400.4}{10.4204/EPTCS.400.4}}
\pdfoutput=1

